More Photos are All You Need: Semi-Supervised Learning for Fine-Grained Sketch Based Image Retrieval

A fundamental challenge faced by existing Fine-Grained Sketch-Based Image Retrieval (FG-SBIR) models is the data scarcity -- model performances are largely bottlenecked by the lack of sketch-photo pairs. Whilst the number of photos can be easily scaled, each corresponding sketch still needs to be individually produced. In this paper, we aim to mitigate such an upper-bound on sketch data, and study whether unlabelled photos alone (of which they are many) can be cultivated for performances gain. In particular, we introduce a novel semi-supervised framework for cross-modal retrieval that can additionally leverage large-scale unlabelled photos to account for data scarcity. At the centre of our semi-supervision design is a sequential photo-to-sketch generation model that aims to generate paired sketches for unlabelled photos. Importantly, we further introduce a discriminator guided mechanism to guide against unfaithful generation, together with a distillation loss based regularizer to provide tolerance against noisy training samples. Last but not least, we treat generation and retrieval as two conjugate problems, where a joint learning procedure is devised for each module to mutually benefit from each other. Extensive experiments show that our semi-supervised model yields significant performance boost over the state-of-the-art supervised alternatives, as well as existing methods that can exploit unlabelled photos for FG-SBIR.

==> Arxiv Semi Supervised/dumping_yard.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[]
    \centering
    \caption{Retrieval Study dummy caption}
    \scriptsize
    \begin{tabular}{c|ccc|ccc}
    % \toprule\toprule
    \hline \hline
         & \multicolumn{3}{c|}{Chair-V2} & \multicolumn{3}{c}{Shoe-V2} \\
        \cline{2-7}
         & Acc.@1 & Acc.@5 & Acc.@10 & Acc.@1 & Acc.@5 & Acc.@10 \\
        % \midrule
        \hline
        Human & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        % \hdashline
        Baseline-1 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-2 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-3 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-4 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        % \hdashline
        Our Proposed & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        % \bottomrule
        \hline
    \end{tabular}
    \label{tab:retrieval}
\end{table}


\setlength{\tabcolsep}{7pt}
\begin{table*}[]
    \centering
    \caption{Generation dummy caption}
    \scriptsize
    \begin{tabular}{c|cc|cc|c|cc|cc|c}
        \toprule\toprule
         & \multicolumn{5}{c|}{Chair-V2} & \multicolumn{5}{c}{Shoe-V2} \\
        \cline{2-11}
         & \multicolumn{2}{c|}{Recognition} & \multicolumn{2}{c|}{Retrieval} & \multirow{2}{*}{FID Score} & \multicolumn{2}{c|}{Recognition} & \multicolumn{2}{c|}{Retrieval} & \multirow{2}{*}{FID Score} \\
         & Acc.@1 & Acc.@5 & Acc.@1 & Acc.@5 &  & Acc.@1 & Acc.@5 & Acc.@1 & Acc.@5 & \\
        \midrule
        Human & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        \hdashline
        Baseline-1 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-2 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-3 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-4 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        \hdashline
        Our Proposed & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        \bottomrule
    \end{tabular}
    \label{tab:generation}
\end{table*}

==> dumping_yard.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[]
    \centering
    \caption{Retrieval Study dummy caption}
    \scriptsize
    \begin{tabular}{c|ccc|ccc}
    % \toprule\toprule
    \hline \hline
         & \multicolumn{3}{c|}{Chair-V2} & \multicolumn{3}{c}{Shoe-V2} \\
        \cline{2-7}
         & Acc.@1 & Acc.@5 & Acc.@10 & Acc.@1 & Acc.@5 & Acc.@10 \\
        % \midrule
        \hline
        Human & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        % \hdashline
        Baseline-1 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-2 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-3 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-4 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        % \hdashline
        Our Proposed & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        % \bottomrule
        \hline
    \end{tabular}
    \label{tab:retrieval}
\end{table}


\setlength{\tabcolsep}{7pt}
\begin{table*}[]
    \centering
    \caption{Generation dummy caption}
    \scriptsize
    \begin{tabular}{c|cc|cc|c|cc|cc|c}
        \toprule\toprule
         & \multicolumn{5}{c|}{Chair-V2} & \multicolumn{5}{c}{Shoe-V2} \\
        \cline{2-11}
         & \multicolumn{2}{c|}{Recognition} & \multicolumn{2}{c|}{Retrieval} & \multirow{2}{*}{FID Score} & \multicolumn{2}{c|}{Recognition} & \multicolumn{2}{c|}{Retrieval} & \multirow{2}{*}{FID Score} \\
         & Acc.@1 & Acc.@5 & Acc.@1 & Acc.@5 &  & Acc.@1 & Acc.@5 & Acc.@1 & Acc.@5 & \\
        \midrule
        Human & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        \hdashline
        Baseline-1 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-2 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-3 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        Baseline-4 & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        \hdashline
        Our Proposed & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% & 99.9\% \\
        \bottomrule
    \end{tabular}
    \label{tab:generation}
\end{table*}
